HIP 33609 b: An Eccentric Brown Dwarf Transiting a V=7.3 Rapidly Rotating B-Star

We present the discovery and characterization of HIP 33609 b, a transiting warm brown dwarf orbiting a late B star, discovered by NASA's Transiting Exoplanet Survey Satellite TESS as TOI-588 b. HIP 33609 b is a large (R$_{b}$ = 1.580$_{-0.070}^{+0.074}$ R$_{J}$) brown dwarf on a highly eccentric (e = 0.560$_{-0.031}^{+0.029}$) orbit with a 39-day period. The host star is a bright (V = 7.3 mag), T$_{eff}$ = 10,400$_{-660}^{+800}$ K star with a mass of M$_{*}$ = 2.383$_{-0.095}^{+0.10}$ M$_{\odot}$ and radius of R$_{*}$ = 1.863$_{-0.082}^{+0.087}$ R$_{\odot}$, making it the hottest transiting brown dwarf host star discovered to date. We obtained radial velocity measurements from the CHIRON spectrograph confirming the companion's mass of M$_{b}$ = 68.0$_{-7.1}^{+7.4}$ M$_{J}$ as well as the host star's rotation rate ($vsini_{*} = 55.6 \pm 1.8$ km/s). We also present the discovery of a new comoving group of stars, designated as MELANGE-6, and determine that HIP 33609 is a member. We use a combination of rotation periods and isochrone models fit to the cluster members to estimate an age of 150 $\pm$ 25 Myr. With a measured mass, radius, and age, HIP 33609 b becomes a benchmark for substellar evolutionary models.

==> rv_table.tex <==
\begin{deluxetable}{l l l}[bt]
\tabletypesize{\scriptsize}
\tablecaption{The radial velocity measurements for the HIP 33609 system.}
\tablewidth{0pt}
\tablehead{
\colhead{\bjdtdb} & \colhead{RV (m s$^{-1}$)} & \colhead{$\sigma_{RV}$ (m s$^{-1}$)}}
\startdata
2458872.64968 & 32201.9 & 769.6 \\
2458874.68716 & 29813.7 & 1029.1 \\
2459265.59795 & 31140.8 & 1125.7 \\
2459271.58653 & 29249.9 & 1019.7 \\
2459276.56080 & 28538.2 & 842.3 \\
2459281.57067 & 30041.5 & 1049.7 \\
2459286.69996 & 33204.2 & 974.2 \\
2459294.55752 & 32251.1 & 1093.2 \\
2459303.54558 & 32293.7 & 1167.0 \\
2459321.52137 & 30560.4 & 900.5 \\
2459323.52343 & 30998.6 & 992.5 \\
2459331.46144 & 31450.3 & 685.8 \\
2459333.48087 & 31801.6 & 1571.2 \\
2459336.46010 & 32079.4 & 868.0 \\
2459340.49478 & 32912.0 & 930.0  \\
2459342.47356 & 31829.6 & 1002.2 \\
2459344.46994 & 32443.8 & 1230.7 \\
2459347.50808 & 31687.2 & 979.7 \\
2459351.46803 & 26993.6 & 1195.5 \\
2459361.44832 & 30419.7 & 591.6 \\
2459364.44268 & 31314.1 & 873.7 \\
2459497.86645 & 32346.2 & 1247.6 \\
2459498.86337 & 33896.8 & 823.9 \\
2459502.88700 & 31873.6 & 702.7 \\
2459505.82903 & 31722.4 & 1189.3 \\
2459506.88278 & 29142.3 & 896.2 \\
2459508.84044 & 29556.2 & 785.5 \\
2459509.76436 & 27200.5 & 998.3 \\
2459510.79825 & 27373.0 & 1564.7 \\
2459511.77084 & 27838.5 & 820.2 \\
2459512.81732 & 27742.1 & 886.0 \\
2459513.82850 & 29202.6 & 853.4 \\
2459514.80241 & 29779.1 & 889.0 \\
2459515.76514 & 30906.6 & 792.1  \\
2459516.81742 & 31576.8 & 917.3  \\
2459517.82665 & 30789.3 & 711.5 \\
2459518.73563 & 31764.7 & 927.9 \\
2459519.81360 & 31232.3 & 1781.9 \\
2459520.79849 & 33014.2 & 944.1 \\
\hline
\enddata
\end{deluxetable}

==> toi588.sed.rv.transit.median.tex <==
\providecommand{\bjdtdb}{\ensuremath{\rm {BJD_{TDB}}}}
\providecommand{\feh}{\ensuremath{\left[{\rm Fe}/{\rm H}\right]}}
\providecommand{\teff}{\ensuremath{T_{\rm eff}}}
\providecommand{\teq}{\ensuremath{T_{\rm eq}}}
\providecommand{\ecosw}{\ensuremath{e\cos{\omega_*}}}
\providecommand{\esinw}{\ensuremath{e\sin{\omega_*}}}
\providecommand{\msun}{\ensuremath{\,M_\Sun}}
\providecommand{\rsun}{\ensuremath{\,R_\Sun}}
\providecommand{\lsun}{\ensuremath{\,L_\Sun}}
\providecommand{\mj}{\ensuremath{\,M_{\rm J}}}
\providecommand{\rj}{\ensuremath{\,R_{\rm J}}}
\providecommand{\me}{\ensuremath{\,M_{\rm E}}}
\providecommand{\re}{\ensuremath{\,R_{\rm E}}}
\providecommand{\fave}{\langle F \rangle}
\providecommand{\fluxcgs}{10$^9$ erg s$^{-1}$ cm$^{-2}$}

\startlongtable
\begin{deluxetable*}{lccc}
\tablecaption{Median values and 68\% confidence interval for toi588.sed.rv.transit.}
\tablehead{\colhead{~~~Parameter} & \colhead{Units} & \multicolumn{2}{c}{Values}}
\startdata
\smallskip\\\multicolumn{2}{l}{Stellar Parameters:}&\smallskip\\
~~~~$M_*$\dotfill &Mass (\msun)\dotfill &$2.26^{+0.19}_{-0.28}$\\
~~~~$R_*$\dotfill &Radius (\rsun)\dotfill &$1.838^{+0.078}_{-0.076}$\\
~~~~$R_{*,SED}$\dotfill &Radius$^{1}$ (\rsun)\dotfill &$1.830^{+0.054}_{-0.057}$\\
~~~~$L_*$\dotfill &Luminosity (\lsun)\dotfill &$38.0^{+11}_{-7.4}$\\
~~~~$F_{Bol}$\dotfill &Bolometric Flux (cgs)\dotfill &$0.0000000511^{+0.000000014}_{-0.0000000100}$\\
~~~~$\rho_*$\dotfill &Density (cgs)\dotfill &$0.506^{+0.091}_{-0.080}$\\
~~~~$\log{g}$\dotfill &Surface gravity (cgs)\dotfill &$4.259^{+0.057}_{-0.063}$\\
~~~~$T_{\rm eff}$\dotfill &Effective Temperature (K)\dotfill &$10570^{+850}_{-710}$\\
~~~~$T_{\rm eff,SED}$\dotfill &Effective Temperature$^{1}$ (K)\dotfill &$10590^{+840}_{-700}$\\
~~~~$[{\rm Fe/H}]$\dotfill &Metallicity (dex)\dotfill &$-0.26^{+0.38}_{-0.61}$\\
~~~~$[{\rm Fe/H}]_{0}$\dotfill &Initial Metallicity$^{2}$ \dotfill &$-0.21^{+0.35}_{-0.58}$\\
~~~~$Age$\dotfill &Age (Gyr)\dotfill &$0.26^{+0.32}_{-0.18}$\\
~~~~$EEP$\dotfill &Equal Evolutionary Phase$^{3}$ \dotfill &$332^{+31}_{-40}$\\
~~~~$A_V$\dotfill &V-band extinction (mag)\dotfill &$0.129^{+0.081}_{-0.084}$\\
~~~~$\sigma_{SED}$\dotfill &SED photometry error scaling \dotfill &$1.30^{+0.39}_{-0.26}$\\
~~~~$\varpi$\dotfill &Parallax (mas)\dotfill &$6.484\pm0.049$\\
~~~~$d$\dotfill &Distance (pc)\dotfill &$154.2\pm1.2$\\
\smallskip\\\multicolumn{2}{l}{Planetary Parameters:}&b\smallskip\\
~~~~$P$\dotfill &Period (days)\dotfill &$39.471813^{+0.000016}_{-0.000017}$\\
~~~~$R_P$\dotfill &Radius (\rj)\dotfill &$1.565^{+0.066}_{-0.065}$\\
~~~~$M_P$\dotfill &Mass (\mj)\dotfill &$67^{+16}_{-15}$\\
~~~~$T_C$\dotfill &Time of conjunction$^{4}$ (\bjdtdb)\dotfill &$2231.75862\pm0.00022$\\
~~~~$T_T$\dotfill &Time of minimum projected separation$^{5}$ (\bjdtdb)\dotfill &$2231.75884\pm0.00021$\\
~~~~$T_0$\dotfill &Optimal conjunction Time$^{6}$ (\bjdtdb)\dotfill &$1994.92773^{+0.00020}_{-0.00019}$\\
~~~~$a$\dotfill &Semi-major axis (AU)\dotfill &$0.3007^{+0.0082}_{-0.013}$\\
~~~~$i$\dotfill &Inclination (Degrees)\dotfill &$89.22\pm0.18$\\
~~~~$e$\dotfill &Eccentricity \dotfill &$0.537^{+0.058}_{-0.061}$\\
~~~~$\omega_*$\dotfill &Argument of Periastron (Degrees)\dotfill &$160.7^{+8.2}_{-9.1}$\\
~~~~$T_{eq}$\dotfill &Equilibrium temperature$^{7}$ (K)\dotfill &$1266^{+78}_{-71}$\\
~~~~$\tau_{\rm circ}$\dotfill &Tidal circularization timescale (Gyr)\dotfill &$13100^{+16000}_{-7900}$\\
~~~~$K$\dotfill &RV semi-amplitude (m/s)\dotfill &$2760^{+590}_{-610}$\\
~~~~$R_P/R_*$\dotfill &Radius of planet in stellar radii \dotfill &$0.08750\pm0.00026$\\
~~~~$a/R_*$\dotfill &Semi-major axis in stellar radii \dotfill &$35.0\pm2.0$\\
~~~~$\delta$\dotfill &Transit depth (fraction)\dotfill &$0.007657^{+0.000045}_{-0.000046}$\\
~~~~$Depth$\dotfill &Flux decrement at mid transit \dotfill &$0.007657^{+0.000045}_{-0.000046}$\\
~~~~$\tau$\dotfill &Ingress/egress transit duration (days)\dotfill &$0.02362^{+0.00088}_{-0.00090}$\\
~~~~$T_{14}$\dotfill &Total transit duration (days)\dotfill &$0.27014^{+0.00090}_{-0.00092}$\\
~~~~$T_{FWHM}$\dotfill &FWHM transit duration (days)\dotfill &$0.24652\pm0.00037$\\
~~~~$b$\dotfill &Transit Impact parameter \dotfill &$0.293^{+0.049}_{-0.065}$\\
~~~~$b_S$\dotfill &Eclipse impact parameter \dotfill &$0.410^{+0.090}_{-0.094}$\\
~~~~$\tau_S$\dotfill &Ingress/egress eclipse duration (days)\dotfill &$0.0352^{+0.0068}_{-0.0052}$\\
~~~~$T_{S,14}$\dotfill &Total eclipse duration (days)\dotfill &$0.368^{+0.046}_{-0.041}$\\
~~~~$T_{S,FWHM}$\dotfill &FWHM eclipse duration (days)\dotfill &$0.332^{+0.040}_{-0.036}$\\
~~~~$\delta_{S,2.5\mu m}$\dotfill &Blackbody eclipse depth at 2.5$\mu$m (ppm)\dotfill &$59^{+12}_{-10.}$\\
~~~~$\delta_{S,5.0\mu m}$\dotfill &Blackbody eclipse depth at 5.0$\mu$m (ppm)\dotfill &$274^{+22}_{-21}$\\
~~~~$\delta_{S,7.5\mu m}$\dotfill &Blackbody eclipse depth at 7.5$\mu$m (ppm)\dotfill &$427^{+23}_{-20}$\\
~~~~$\rho_P$\dotfill &Density (cgs)\dotfill &$21.6^{+6.2}_{-5.5}$\\
~~~~$logg_P$\dotfill &Surface gravity \dotfill &$4.831^{+0.100}_{-0.12}$\\
~~~~$\Theta$\dotfill &Safronov Number \dotfill &$11.6\pm2.6$\\
~~~~$\fave$\dotfill &Incident Flux (\fluxcgs)\dotfill &$0.445^{+0.13}_{-0.095}$\\
~~~~$T_P$\dotfill &Time of Periastron (\bjdtdb)\dotfill &$2194.63^{+0.44}_{-0.40}$\\
~~~~$T_S$\dotfill &Time of eclipse (\bjdtdb)\dotfill &$2239.2^{+1.6}_{-1.4}$\\
~~~~$T_A$\dotfill &Time of Ascending Node (\bjdtdb)\dotfill &$2220.1^{+1.7}_{-1.9}$\\
~~~~$T_D$\dotfill &Time of Descending Node (\bjdtdb)\dotfill &$2195.23^{+0.56}_{-0.48}$\\
~~~~$V_c/V_e$\dotfill & \dotfill &$0.718\pm0.042$\\
~~~~$e\cos{\omega_*}$\dotfill & \dotfill &$-0.503^{+0.076}_{-0.071}$\\
~~~~$e\sin{\omega_*}$\dotfill & \dotfill &$0.175^{+0.067}_{-0.068}$\\
~~~~$M_P\sin i$\dotfill &Minimum mass (\mj)\dotfill &$67^{+16}_{-15}$\\
~~~~$M_P/M_*$\dotfill &Mass ratio \dotfill &$0.0289^{+0.0062}_{-0.0063}$\\
~~~~$d/R_*$\dotfill &Separation at mid transit \dotfill &$21.2^{+3.1}_{-2.8}$\\
~~~~$P_T$\dotfill &A priori non-grazing transit prob \dotfill &$0.0431^{+0.0066}_{-0.0054}$\\
~~~~$P_{T,G}$\dotfill &A priori transit prob \dotfill &$0.0514^{+0.0079}_{-0.0065}$\\
~~~~$P_S$\dotfill &A priori non-grazing eclipse prob \dotfill &$0.0301^{+0.0050}_{-0.0037}$\\
~~~~$P_{S,G}$\dotfill &A priori eclipse prob \dotfill &$0.0358^{+0.0060}_{-0.0044}$\\
\smallskip\\\multicolumn{2}{l}{Wavelength Parameters:}&TESS\smallskip\\
~~~~$u_{1}$\dotfill &linear limb-darkening coeff \dotfill &$0.1798\pm0.0087$\\
~~~~$u_{2}$\dotfill &quadratic limb-darkening coeff \dotfill &$0.2410\pm0.0096$\\
~~~~$A_D$\dotfill &Dilution from neighboring stars \dotfill &$-0.0000\pm0.0016$\\
\smallskip\\\multicolumn{2}{l}{Telescope Parameters:}&chiron\smallskip\\
~~~~$\gamma_{\rm rel}$\dotfill &Relative RV Offset (m/s)\dotfill &$32890\pm230$\\
~~~~$\sigma_J$\dotfill &RV Jitter (m/s)\dotfill &$280^{+420}_{-280}$\\
~~~~$\sigma_J^2$\dotfill &RV Jitter Variance \dotfill &$80000^{+410000}_{-220000}$\\
\smallskip\\\multicolumn{2}{l}{Transit Parameters:}&TESS UT oi58-8_-ql (TESS)&TESS UT oi58-8_-sp (TESS)\smallskip\\
~~~~$\sigma^{2}$\dotfill &Added Variance \dotfill &$-0.0000009725^{+0.0000000029}_{-0.0000000023}$&$0.0000000282^{+0.0000000050}_{-0.0000000046}$\\
~~~~$F_0$\dotfill &Baseline flux \dotfill &$0.999974\pm0.000017$&$1.000001\pm0.000012$\\
\enddata
\label{tab:toi588.sed.rv.transit.}
\tablenotetext{}{See Table 3 in \citet{Eastman:2019} for a detailed description of all parameters}
\tablenotetext{1}{This value ignores the systematic error and is for reference only}
\tablenotetext{2}{The metallicity of the star at birth}
\tablenotetext{3}{Corresponds to static points in a star's evolutionary history. See \S2 in \citet{Dotter:2016}.}
\tablenotetext{4}{Time of conjunction is commonly reported as the "transit time"}
\tablenotetext{5}{Time of minimum projected separation is a more correct "transit time"}
\tablenotetext{6}{Optimal time of conjunction minimizes the covariance between $T_C$ and Period}
\tablenotetext{7}{Assumes no albedo and perfect redistribution}
\end{deluxetable*}

